The large-scale monopole of the power spectrum in a Euclid-like survey: wide-angle effects, lensing, and the `finger of the observer'

Radial redshift-space distortions due to peculiar velocities and other light-cone effects shape the maps we build of the Universe. We address the open question of their impact onto the monopole moment of the galaxy power spectrum, $P_0(k)$. Specifically, we use an upgraded numerical implementation of the LIGER method to generate $140$ mock galaxy density fields for a full Euclid-like survey and we measure $P_0(k)$ in each of them utilising a standard estimator. We compare the spectra obtained by turning on and off different effects. Our results show that wide-angle effects due to radial peculiar velocities generate excess power above the level expected within the plane-parallel approximation. They are detectable with a signal-to-noise ratio of 2.7 for $k<0.02\,h$ Mpc$^{-1}$. Weak-lensing magnification also produces additional power on large scales which, if the current favourite model for the luminosity function of H$\alpha$ emitters turns out to be realistic, can only be detected with a signal-to-noise ratio of 1.3 at best. Finally, we demonstrate that measuring $P_0(k)$ in the standard of rest of the observer generates an additive component reflecting the kinematic dipole overdensity caused by the peculiar velocity. This component is characterised by a damped oscillatory pattern on large scales. We show that this `finger of the observer' effect is detectable in some redshift bins and suggest that its measurement could possibly open new research directions in connection with the determination of the cosmological parameters, the properties of the galaxy population under study, and the dipole itself.

==> misc.tex <==
@COMMENT{
% @ARTICLE{CLASSIII,
%       author = {{Lesgourgues}, Julien},
%         title = "{The Cosmic Linear Anisotropy Solving System (CLASS) I: Overview}",
%       journal = {arXiv e-prints},
%      keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
%          year = 2011,
%         month = apr,
%           eid = {arXiv:1104.2932},
%         pages = {arXiv:1104.2932},
% archivePrefix = {arXiv},
%       eprint = {1104.2932},
%  primaryClass = {astro-ph.IM},
%       adsurl = {https://ui.adsabs.harvard.edu/abs/2011arXiv1104.2932L},
%       adsnote = {Provided by the SAO/NASA Astrophysics Data System}
% }
}%\begin{figure}
%    \centering
%	\includegraphics[width=0.4\textwidth]{figs/CHI_LENSING.pdf}
%    \caption{\MYK{\textbf{Top}: The spectra of the models considered in the statistical test shown in the bottom panel.
%    \textbf{Bottom}: A histogram of the number of realizations which result in a particular value of $\Delta \chi^2$, There are 140 realizations in each panel, The histograms are binned at $\Delta \chi^2=1$.}}
%    \label{fig:All_chi_squared}
%\end{figure}
% \subsection{Integral constraint}
% We then compute the recompute the OBS spectra using the "true`` comoving density, which is the average of the comoving density of all the realizations. The $\bar(n)$ has a slight boost in power at large scales for all redshifts, the redshift bin with the strongest effect is shown in  \cref{fig:constraint}, .  
% \begin{figure}
%     \centering
% 	\includegraphics[width=0.3\textwidth]{figs/TNBAR110.pdf}
%     \caption{\MYK{The OBS spectra computed using each realization's density $\hat{n}$ are plotted compared to the spectra computed using the "true`` density $\bar{n}$.}}
%     \label{fig:constraint}
% \end{figure}
    % \item wide angle effects in ratio plots \cref{fig:ratio}
    % Next we test if the Kaiser boost can predict the shift in the $v_r$ spectra, we compute the $v_r$ and realspace galaxy spectra for a fullsky survey , Euclid-like survey and a $10^2 deg^2$ square patch in the sky. The ratio between the $v_r$ and galaxy spectra for all three surveys are shown in \cref{fig:ratio} as well as the Kaiser prediction with/without neglecting the $\alpha = \frac{\dif \ln r^2 \bar{n}}{\dif \ln r}$. As seen in the figure, the ratio exceeds the Kaiser limit at large scales. This increase in the ratio seems to be proportional to the size of the survey. The most likely explanation of this behavior is wide angle effects. The estimator for the monopole of the power spectrum does not include the plane parallel approximation while the Kaiser limit is derived under that assumption. We hypothesis that due to the size of the survey, this assumption falls on large scales.

% \end{itemize}
% \item window function
% \begin{itemize}
%     \item Realspace and vRSD fullsky with convolved window plots \cref{fig:ratio}
%     To find the effect of the window function, we use \cref{eq:obs_power} to compute the $P_{\mathrm{obs}}$ for the galaxy and $v_{\mathrm{r}}$ spectra, we use the average angular comoving density of each realization to compute its spectrum to put the integral constraint term to zero. We use \ts{camb}\cite{CAMBS} to compute the Dark matter power spectrum and we calculate the amplitude of the spectrum for our wide redshift bins using the integral in \cite{Yamamoto_LC} with the bias The Kaiser terms for the galaxy and $v_r$ spectrum respectively. We then convolved the model spectra with the window function for fullsky survey. As seen in \cref{fig:fullsky_wind}, The window function flattens the power spectrum at large scales which is seen in the in the model spectrum The \ts{liger} produced spectra of the galaxy light cones. The $v_r$ light cone spectra is boosted from the Kaiser predicted model -most likely- due to wide angel effects.
% %         \begin{figure*}
% %     \centering
% % 	\includegraphics[width=1\textwidth]{figs/p_spec_fullsky_paper_nbar_all_shades.png}
% %     \caption{The spectra for $v_r$ and galaxy light cones for a fullsky survey compared to the model spectra before and after convoloving with the window function.}
% %     \label{fig:fullsky_wind}
% % \end{figure*}
% \end{itemize}
% \item integral constraint
%     \begin{itemize}
%     \item GRRSD vRSD,vMAG realspace comparison for euclid only but with the averaged nbar to see difference (Maybe plot together with individual nbar ) \cref{fig:constraint}

% % \item covariance matrix
% \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/Hist_delta_chi_kaiser.pdf}
%     \caption{}
%     \label{fig:chi_OBS}
%     \end{figure*}
%             \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/Hist_delta_chi_wideangle.pdf}
%     \caption{}
%     \label{fig:P_OBs}
%     \end{figure*}
% \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/Hist_delta_chi_lensing4.pdf}
%     \caption{}
%     \label{fig:chi_OBS_kaiser}
%     \end{figure*}
%             \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/Hist_delta_chi_lensing1.pdf}
%     \caption{}
%     \label{fig:P_OBs_kaiser}
%     \end{figure*}
%                 \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/BIGbing dist.pdf}
%     \caption{Distribution of $\Delta \chi ^2$ of the big lensing bin }
%     \label{fig:P_OBs_kaiser}
%     \end{figure*}
%                 \begin{figure*}
%     \centering
% 	\includegraphics[width=0.9\textwidth]{figs/scatter_plot_vel_pspec.pdf}
%     \caption{}
%     \label{fig:P_OBs_kaiser}
%     \end{figure*}
% \end{itemize}

%     \begin{itemize}
%     \item GRRSD vRSD with their observor counter part \cref{fig:obs_vel}
%     We finally test how the observer velocity and potential affect the power spectra. As seen in \cref{fig:obs_vel}, the observer information only changes the power spectra at the first few bins both for the $v_r$ The GR spectra.

% \end{itemize}

% \end{enumerate}

______________________________________________________________________
% \section{Validation against \textsc{CLASS}}
% %\section{\ts{liger} Confirmation study.}
% %To measure how realistic the \ts{liger} mocks are, we need to choose a statistic. 
% %In order to coompare the \ts{liger} mocks with theoritical predictions ble to reproduce the theoretical res We present in this section a comparison between \ts{liger} and the code CLASS \citep{CLASSI,CLASSII}
% In order to measure how accurately the \ts{liger} mocks reproduce the expected statistical properties, we measure the angular power spectra for the \ts{liger} mocks and compare them with the theoretical spectra obtained using CLASS \citep{CLASSI,CLASSII}. The choice of the angular power spectra allows us to measure the accuracy of the \ts{liger} mocks in both  configuration shift  and redshift space. %However, it should be emphasized that
% \footnote{The \ts{liger} outputs the density fields which gives the user the freedom to measure the any statistic of interest under the assumption that an estimator can be written.}
% \subsection{$C_{\ell}$ estimation in \ts{liger}.}
% Our inputs are DM-only simulation, consequently we have the interpolated density for each galaxy distribution not the particles themselves \citep{\ts{liger}}.To estimate the interpolated density, we paint the densities in a cubic box of $ L_{\mathrm{box}}=8\,h^{-1}$ Gpc which is slightly larger than the diameter of the light cone with a $512^3$ grid. Increasing the volume of the enclosing cube does not provide any advantage for the estimation of the angular power spectrum. Later in the 3D power spectrum estimation, we use roughly twice that size to probe higher scales \footnote{Having a larger cube decreases the fundamental frequency of the box probing more large scales.}
% We then create digitized sky maps using HEALPix \citep{HEALpix} with $N_{\mathrm{pix}}=2\times(512)^2$. We  measure the projected number density contrast on the sky using using  \citep{C_LEST}
% \begin{equation}\
% \label{C_L_INTEGRAL}
% \sigma(\Omega)\, = \, \int_0^{\infty}\Phi(r) \frac{n(\mathbf{r})}{\bar{n}(r)}\,r^2 \dif r -1.
% \end{equation}
% $\Phi(r) \propto W(r) n_g(r)$ where $W(r)$ is the window function and is normalized such that $\int \Phi(r) r^2 \dif r = N/4\pi$ with $N$ as the total number of galaxies.% The window function contains the redshift information, our implementation was a tophat function which zeroed the densities outside of the redshift range of interest.

% To compute \cref{C_L_INTEGRAL}, we use the Fast voxel Traversal Algorithm for Ray tracing \citep{RAY} to calculate the line integral on a $1024^3$ grid to the center of each pixel of the HEALpix maps. The redshift range is defined by the window function in $W(r)$. We use a tophat function which zeros the densities outside of the redshift range of interest. We then decompose the maps into spherical harmonics
% \begin{equation}
% a_{\ell m}=\int d\Omega\, \sigma(\Omega)\, Y^*_{\ell m} \,,
% \end{equation}
% and measure the angular auto correlation spectra using 
% \begin{equation}
% \hat{C}_{\ell}=\frac{1}{w_p^{2}(2\ell + 1)}\sum_{m=-\ell}^l |a_{\ell m}|^2 \,-\frac{4\pi}{N} \,,
% \end{equation}
% where $w_p$ is a correction factor of the order unity due to the finite resolution of HEALPix.
% We estimated the auto-correlation spectra in four redshift bins as in \citet{EuclidVII} for 144 fullsky mocks with the Euclid co moving number density shown in \ref{Fig:functions}. To be able to compare with CLASS, we used a constant linear bias 1 for these mocks and a constant magnification bias (Q = 0). For the CLASS spectra, we use the same cosmological parameters previously mentioned, the Euclid comoving number density for both the selection function and the evolutionary bias , $b=1$ and finally $s=0$ \footnote{The parametrization of the magnification bias is slightly difference between CLASS and this work. They are related by $Q=-5/2$}.  The first two bins of the spectra along with the residual error are shown in \cref{fig:ANG_SPEC}.
% \begin{figure*}
% \includegraphics[width=2\columnwidth, keepaspectratio=true]{figs/CL_AND_RATIO.pdf}
% \caption{The angular spectra estimated from \ts{liger} and CLASS are shown in the top panel while the percent difference is plotted in the bottom panel for two redshift bins . In the top panel,The \ts{liger} spectra are shown with stars with error bars given by the standard deviation over 144 mock, binned with $\dif \ell =10$.The CLASS spectra are shown with the dashed lines. In both panels, The blue lines are in configuration space with $b=1$. The red lines are in redshift space after adding all relativistic effects  with the same linear bias and magnification bias $Q=0$.}
% \label{fig:ANG_SPEC} 
% \end{figure*}.

% In \cref{fig:ANG_SPEC}, \ts{liger} agrees well (up to $1\%$) with CLASS up to $\ell=85$ except for the first bin  in real space. The loss of power in the higher $\ell$s could be explained by the limited resolution of the simulation and the interpolation grid. This is supported by the increase in the agreement range with redshift. Increasing the resolution of the original simulation before using \ts{liger} should increase this cutoff. For this work, we are only interested in the large scales, so this should be sufficient for our needs.


%Finally, We compare the effect of neglecting Lensing and the velocity shifts in the spectra for both \ts{liger} and CLASS. As seen in \cref{fig:DCL}, The velocity effects are well traced by \ts{liger}. The lensing on the other hand is well traced in the higher redshift bins, in the first bin becomes smaller than $10^{-2}$, so it's only seen in \ts{liger} in the first few bins. However in the higher redshift bins were the effect is stronger the lensing is well traced up to the resolution cutoff.
%\begin{figure}
%\includegraphics[width=1\columnwidth, keepaspectratio=true]{figs/ANG_DCL.pdf}
%\caption{The fractional difference between the full Red shift spectra and the spectra computed after neglecting lensing in red and the all RSD effects in blue. The \ts{liger} spectra is given by the triangles binned with $\dif \ell=10$ while class is shown with the bold lines.}
%\label{fig:DCL} 
%\end{figure}.
_____________________________________________________________________
___________________________________________________________________
